Discriminating image representations with principal distortions

Image representations (artificial or biological) are often compared in terms of their global geometric structure; however, representations with similar global structure can have strikingly different local geometries. Here, we propose a framework for comparing a set of image representations in terms of their local geometries. We quantify the local geometry of a representation using the Fisher information matrix, a standard statistical tool for characterizing the sensitivity to local stimulus distortions, and use this as a substrate for a metric on the local geometry in the vicinity of a base image. This metric may then be used to optimally differentiate a set of models, by finding a pair of "principal distortions" that maximize the variance of the models under this metric. As an example, we use this framework to compare a set of simple models of the early visual system, identifying a novel set of image distortions that allow immediate comparison of the models by visual inspection. In a second example, we apply our method to a set of deep neural network models and reveal differences in the local geometry that arise due to architecture and training types. These examples demonstrate how our framework can be used to probe for informative differences in local sensitivities between complex models, and suggest how it could be used to compare model representations with human perception.

==> body.tex <==
\section{Introduction}

Biological and artificial neural networks transform sensory stimuli into internal representations that support downstream tasks. 
% \comment{
% The geometry of these high-dimensional representations is often reported to be similar across systems \citep{zhang2018unreasonable,chung2021neural,huh2024platonic}. Yet, other work has suggested stark differences between biological systems and computational models. Here, we propose a metric on image representations that can be used to characterize differences in their local geometries.}
%
Often, similarity between representations is quantified by measuring the alignment of their \textit{global} geometric structure \citep{kriegeskorte2008representational,yamins2016using,raghu2017svcca,kornblith2019similarity,williams2021generalized}.
%These global measures focus on the structure of responses to natural stimuli that are relatively far away in input space (e.g., images of different objects). 
However, systems with similar global geometry can have strikingly different \textit{local} geometries.
The well-known occurrence of adversarial examples \citep{szegedy2013intriguing,goodfellow2014explaining} in object recognition systems provides an example: Even for systems that are broadly similar to each other and in agreement with human perception, carefully targeted experiments reveal small image distortions that are imperceptible to humans but result in reliable misclassification by a model.

% For example, \citet{szegedy2013intriguing} found image distortions that were imperceptible to humans but led artificial neural networks to misclassify images, leading to ways of training artificial neural networks to reduce these adversarial examples \citep{goodfellow2014explaining, madry2017towards}. Even though these models seem similar to standard models when evaluated with natural images, they have representations that are more aligned with humans for images off of the natural manifold \cite{harringtonfinding, feather2023model, gaziv2023robustified}. However, even within these more aligned models, it remains unclear which type of model should be further investigated, because there are many different types of adversarial training or ways to incorporate biologically inspired architectural motifs that seem to yield similar results with existing methods. 

% Taken together, these observations suggest a need for metrics that compare the local geometries of image representations across both artificial neural networks and the human visual system and, in particular, highlight the differences between systems.

How can we quantify and compare the local geometry of different image representations? A brute-force comparison clearly is prohibitive:
the space of images is extremely high-dimensional, and the set of potential distortions equally high-dimensional.
% For example, estimating the local geometry of the image representation in a human visual system amounts to performing psychophysical experiments estimating the sensitivity of a human subject to small image distortions.
Estimating the local geometry of representations over a moderately dense sampling of this full set is impractical, and estimating human sensitivity to such a set is essentially impossible.
As such, it is worthwhile to develop a method for judicious selection of stimulus distortions that can be used when comparing a set of models.
% As such, it is worthwhile to develop a measure of local distortion sensitivity, and to use this to optimize the judicious selection of stimuli that can be used in comparing a set of models.

We take inspiration from \citet{zhou2024comparing}.
For a pair of models and a base image, they synthesize distortions along which the two models' sensitivities maximally disagree. This bears conceptual similarity to other methods that construct stimuli to optimally distinguish models \citep{wang2008maximum,golan2020controversial}, and builds on earlier work that examined ``eigen-distortions'' along which individual models are maximally/minimally sensitive \citep{berardino2017eigen}.
Specifically, they measure the local sensitivity of a model in terms of its Fisher Information matrix (FIM) \citep{fisher1925theory}, a classical tool from statistical estimation theory, and choose the pair of ``generalized eigen-distortions'' that maximize/minimize the ratio of the two models' sensitivities.
% The sensitivity of an image representation to local distortions can be computed in terms of the Fisher Information matrix (FIM) \citep{fisher1925theory}, a classical tool from statistical estimation theory.
% The FIM has been previously proposed as a substrate for model comparison.  To compare the local sensitivities of a pair image representations about a given image, \citet{zhou2024comparing} proposed the use of two ``generalized eigen-distortions'' along which the ratio of FIM-determined sensitivities of the two models is maximized/minimized.
% This built on earlier work \citep{berardino2017eigen} which examined ``eigen-distortions'' along which individual models are maximally/minimally sensitive.
% , and bears conceptual similarity to other methods that construct stimuli to optimally distinguish models \citep{wang2008maximum,golan2020controversial}.
Once these image distortion have been computed, they may be added in varying amounts to a base image to determine the level at which they become visible to a human.  These measured human sensitivities can then be compared to those of the models, with the goal of identifying which model is better aligned with the local geometry of the human visual system.
% However, two significant challenges remain.
% First, given measurements of human sensitivities, it is not obvious how to identify which model is better aligned with the human visual system.
However, when comparing more than two models, there is no principled method for selecting the distortions.

\begin{figure}
  \centering
  \includegraphics[width=\textwidth]{figs/Fig1_Sharing_V5.pdf}
  \caption{\small 
  Comparing the local geometry of image representations.
  {\bf A)}
  Each model maps a stimulus $\rvs$ to a distribution $p(\rvr|\rvs)$ in representation space (we assume stochastic representations, as is true of biological neurons, while deterministic models can be consistently measured by assuming additive Gaussian response noise).
  Classical signal detection theory posits that the sensitivity $d(\vepsilon)$ of the representation to a distortion $\vepsilon$ depends on how much overlap there is between $p(\rvr|\rvs)$ and $p(\rvr|\rvs+\vepsilon)$, with less overlap indicating higher sensitivity.
  % Here, responses of three models $A,B,C$ to two distortions $\vepsilon_1,\vepsilon_2$ are shown.
  {\bf B)} Distortion sensitivity of each model may be mapped back to the stimulus domain via the FIM, which has been used previously to generate optimal stimuli for comparison to human perception.  Specifically, the eigenvectors of a model FIM may be used to examine most/least model-sensitive stimuli \citep{berardino2017eigen}, and the generalized eigenvectors of the ratio of model FIMs may be used to generate stimuli that best distinguish the sensitivities of two models \citep{zhou2024comparing}.
  Here, we show that these models have interpretations in terms of the log ratios of model sensitivities, and develop a generalized method that allows comparison of an arbitrary number of models, by selecting two stimulus distortions that maximize the variance of the log-ratio of sensitivities over models.}
  \label{fig:schematic}
  \vspace{-0.2cm}
\end{figure}
% If a computational model is proposed as a possible hypothesis for the computations in the human visual system, we can use it to determine which directions to probe to validate or invalidate the model. 
% Even when the image representation corresponds to a computational model, comprehensive comparisons are computationally intensive and inefficient.
% Therefore, we need a method for efficiently selecting distortions along which to compare local geometries.
% One approach is to find distortions along which the representation of a computational model maximally differs \cite{berardino2017eigen}. If two models are proposed, one can choose distortions that maximize the separation between the models \cite{zhou2024comparing}. 
% This is related to a body of literature on constructing stimuli that directly  differentiate models \citep{wang2008maximum,golan2020controversial,zhou2024comparing}. 
% However, in both cases, the number of different distortions quickly grows when there are many models, and the choice of how to generate stimuli simultaneously from many models has remained unclear. 

Here we define a novel metric for comparing model representations in terms of their sensitivities to a pair of local image distortions. 
We propose using this metric to efficiently generate distortions that maximize the variance of two or more models.
In analogy with principal component analysis, 
% our method can be viewed as a dimensionality reduction technique that preserves as much of the variability in the local representational geometry as possible.  As such, 
we refer to these as ``principal distortions''. 
% These distortions can be used for psychophysical tests to determine which of a set of models best captures the sensitivity of the human visual system.
We apply our method to a nested set of hand-crafted models of the early visual system, and to a set of standard and adversarially-trained visual neural network models. In both cases, we illustrate how the method generates novel distortions that highlight differences between models.

% Perhaps emphasize that our approach compares representations in \textit{stimulus} space, whereas most other approaches directly compare representations.

% How do we compare image representations in terms of their ability to explain human perception?
% One of the most reliable measurements of human perception is stimulus discrimination.
% The goal of this work is to develop a metric for comparing image representations and human perception in terms of stimulus discrimination thresholds.

% Our main contributions are:
% \begin{itemize}
%     \item Given a set of sensitivities to distortions, we define a metric on stochastic image representations.
%     \item We propose a method for selecting distortions to maximally separate models according to the metric, allowing for comparisons across multiple models.
%     % \item Given two distortions of the input, we define a metric between stochastic model representations that relates to the model discrimination thresholds for the distortions.
%     % \item We develop a method to choose the two distortion directions that will maximally separate the models. 
%     % \item We develop a framework to relate the model distortions to human perceptual discrimination thresholds to choose which model is the best description of human visual perception. 
%     \item We apply our method to a set of hierarchical hand-designed models of the early visual system, and to a set of adversarially trained visual neural network models. In both cases, we illustrate how the distortions provide a prediction for which model best captures human visual perception. 
%     % \item We apply our method to a set of adversarially trained models to identify which type of adversarial training results in better alignment with human perceptual discrimination thresholds. 
% \end{itemize}

% \citet{berardino2017eigen} developed a method for comparing image representations in terms of their ability to explain perceptual sensitivity in humans.
% Given such a representation, they compared the eigenvectors of the Fisher information matrix with the largest and smallest eigenvalues, termed ``eigen-distortions'', which correspond to the model-predicted most- and least- noticeable image distortions.
% However, two or more models may share maximal and minimal distortion directions yet produce vastly different perceptual predictions, suggesting that they may not be the optimal image distortions for comparing the perceptual implications of two image representations.

% \citet{zhou2024comparing} proposed a related method for directly comparing two models. 
% By computing the image distortions that maximize (or minimize) the Rayleigh quotient of the Fisher information matrices corresponding to two models, they obtained distortions that maximally differentiate two models.
% However, their method is limited to pairwise comparisons of models.
% Therefore, to compare $N>2$ models, their method requires comparing discrimination thresholds in response to $O(N^2)$ distortions.
% When these distortions are to be tested on human subjects, this can cost significant resources.
% Furthermore, comparing a family of models that are parameterized by a continuous variable is intractable.

% In this study, we generalize the works \citep{berardino2017eigen,zhou2024comparing} by computing the distortion that maximally differentiates any number of image representations in terms of their ability to explain human perceptual sensitivity.
% Given a family image representations, we seek the distortion that maximally differentiates the models in terms of their predicted discrimination thresholds.

% Other related work: \citet{ding2023information} compute the Fisher information of a CNN trained to match the first and second order statistics of salamander retinal responses.

\comment{
Image representations are generally compared in terms of the global geometric properties.
However, image representations with shared global structure may have very different local geometries---e.g., different sensitivities to small distortions
(linear perturbations)
---and these differences can have important practical consequences.
Quantifying differences between local representational geometries is challenging due to the huge number of potential image distortions. 
One approach is to select a small number of image distortions that highlight where the local geometries maximally disagree.
When comparing two representations, optimal selection of the image distortions can be formulated as a generalized eigenvalue problem. 
But it is not clear how to quantify the difference between representations given these distortions and, moreover, there is no systematic method for selecting distortions when comparing more than two representations.
Here, we show that the generalized eigenvalue problem can be reformulated in such a way that it defines a metric between image representations, which quantifies the differences between representations and suggests a natural extension for selecting image distortions when comparing more than two image representations.
}

Global geometry of (visual) representations \citep{kriegeskorte2008representational,kornblith2019similarity,williams2021generalized}.

The local geometries of representations within deep neural networks can be strikingly different from human representations \citep{szegedy2013intriguing,goodfellow2014generative}.
But also, deep networks as perceptual metrics \citep{zhang2018unreasonable}.
Here, we're not asking if deep networks are good models of human visual perception.
Rather, we're asking how models differ in terms of human visual perception.
Global/local structure \citep{muttenthaler2024improving}.

Comparison/competition of models:  \citet{wang2008maximum} (MAD Competition).  Adversarial examples. Controversial stimuli \citet{golan2020controversial}.  
\citet{zhou2024comparing}- generalized eigendistortions.

Human perceptual discrimination thresholds are one of the most reliable methods for probing the local geometry of human visual representations CITE.
However, comprehensive measurements of human discrimination thresholds is impossible for high-dimensional images.
Therefore, we need a method for systematically choosing image distortions.

Eigen-distortions \citep{berardino2017eigen} and generalized eigen-distortions \citep{zhou2024comparing} are methods for evaluating single image representations and comparing two image representations, respectively.
However, it is not clear how to choose image representations to differentiate multiple models.

Here we define a metric for comparing image representations in terms of perceptual discrimination thresholds.
We use this metric to choose image distortions that maximize the pairwise distances between image representations.
In analogy with principal component analysis, our method can be viewed as a dimensionality reduction technique that preserves as much variance as possible.
We compute distances in projected space.

% How do we compare image representations in terms of their ability to explain human perception?
% One of the most reliable measurements of human perception is stimulus discrimination.
% The goal of this work is to develop a metric for comparing image representations and human perception in terms of stimulus discrimination thresholds.

Our main contributions are:
\begin{itemize}
    \item Given a set of distortions, we define a metric on stochastic model representations in terms of their predicted discrimination thresholds.
    \item We propose a method for selecting distortions to maximally separate models according to the metric. Because we are using a metric, we can easily extend to the case of many models. 
    \item We develop a framework to relate the model distortions to human perceptual discrimination thresholds to choose which model is the best description of human visual perception. 
    \item We apply our method to a set of hierarchical hand-designed models of the early visual system (models in \citep{berardino2017eigen}). 
    \item We apply our method to a set of adversarially trained models to identify which type of adversarial training results in better alignment with human perceptual discrimination thresholds. 
\end{itemize}

% Another way to characterize the principal distortions when the noise model is Gaussian: find $\vepsilon_1$, $\vepsilon_2$ that maximizes the variance of
% \begin{align*}
%     \left\{\log\frac{\|f_1(\rvs+\vepsilon_1)-f_1(\rvs)\|}{\|f_1(\rvs+\vepsilon_2)-f_1(\rvs)\|},\dots,\log\frac{\|f_N(\rvs+\vepsilon_1)-f_N(\rvs)\|}{\|f_N(\rvs+\vepsilon_2)-f_N(\rvs)\|}\right\}
% \end{align*}
% This metric is invariant to scaling by a constant $f(\cdot)\mapsto\alpha f(\cdot)$ and to permutation of $\vepsilon_1$ and $\vepsilon_2$.

% \citet{berardino2017eigen} developed a method for comparing image representations in terms of their ability to explain perceptual sensitivity in humans.
% Given such a representation, they compared the eigenvectors of the Fisher information matrix with the largest and smallest eigenvalues, termed ``eigen-distortions'', which correspond to the model-predicted most- and least- noticeable image distortions.
% However, two or more models may share maximal and minimal distortion directions yet produce vastly different perceptual predictions, suggesting that they may not be the optimal image distortions for comparing the perceptual implications of two image representations.

% \citet{zhou2024comparing} proposed a related method for directly comparing two models. 
% By computing the image distortions that maximize (or minimize) the Rayleigh quotient of the Fisher information matrices corresponding to two models, they obtained distortions that maximally differentiate two models.
% However, their method is limited to pairwise comparisons of models.
% Therefore, to compare $N>2$ models, their method requires comparing discrimination thresholds in response to $O(N^2)$ distortions.
% When these distortions are to be tested on human subjects, this can cost significant resources.
% Furthermore, comparing a family of models that are parameterized by a continuous variable is intractable.

% In this study, we generalize the works \citep{berardino2017eigen,zhou2024comparing} by computing the distortion that maximally differentiates any number of image representations in terms of their ability to explain human perceptual sensitivity.
% Given a family image representations, we seek the distortion that maximally differentiates the models in terms of their predicted discrimination thresholds.

% Other related work: \citet{ding2023information} compute the Fisher information of a CNN trained to match the first and second order statistics of salamander retinal responses.

\section{Local geometry of image representations}

Perceptual discriminability is a measure of how well an observer can detect differences between an image $\rvs\in\R^D$ and a small distortion of the image $\rvs+\vepsilon\in\R^D$.
We assume that the observer judges differences based on the stochastic responses $\rvr\in\R^N$ of $N$ neurons.
The \textit{discriminability} between $\rvs$ and $\rvs+\vepsilon$ boils down to computing the mean log likelihood ratio 
 between $p(\rvr|\rvs)$ and $p(\rvr|\rvs+\vepsilon)$, which is approximately
\begin{align*}
    d(\rvs;\vepsilon):=\sqrt{\vepsilon^\top\mI(\rvs)\vepsilon}
\end{align*}
where 
$\mI(\rvs)$ is the Fisher information matrix at $\rvs$ \citep{fisher1925theory}:
\begin{align*}
    \mI(\rvs):=\E\left[\nabla_{\rvs}\log p(\rvr|\rvs)^\top\nabla_{\rvs}\log p(\rvr|\rvs)\right],
\end{align*}
the expectation is over $p(\rvr|\rvs)$ and $\nabla_\rvs\log p(\rvr|\rvs)$ denotes the Jacobian of $\log p(\rvr|\rvs)$ with respect to $\rvs$.
Since discriminability is inversely proportional to discrimination thresholds, the inverse of $d(\rvs;\vepsilon)$ provides an estimate of discrimination thresholds up to a scalar multiple \citep{series2009homunculus}.

% This can all be made mathematically precise.
% Specifically, using the Cram\'er-Rao lower bound, \citet{series2009homunculus} showed that the discrimination threshold at $\rvs$ in the direction $\vepsilon$ for any observer is lower bounded by $\beta t(\rvs;\vepsilon)$, where $\beta$ is a scalar that does not depend on $\rvs$ or $\vepsilon$, $t(\rvs;\vepsilon)$ is the threshold function defined by
% \begin{align}\label{eq:thresh}
%     t(\rvs;\vepsilon):=\sqrt{\vepsilon^\top\mI^{-1}(\rvs)\vepsilon},
% \end{align}
% and $\mI(\rvs)$ is the Fisher information matrix at $\rvs$ \citep{fisher1925theory}:
% \begin{align*}
%     \mI(\rvs):=\E\left[\nabla_{\rvs}\log p(\rvr|\rvs)^\top\nabla_{\rvs}\log p(\rvr|\rvs)\right].
% \end{align*}
% Therefore, given any (stochastic) image representation $p(\rvr|\rvs)$ and an ideal observer that achieves the Cram\'er-Rao lower bound, the threshold function $t(\rvs;\vepsilon)$ provides an estimate of discrimination thresholds up to a scalar multiple.

As an example, suppose that the conditional response $\rvr$ is Gaussian with stimulus-dependent mean $\vmu(\rvs)$ and constant covariance $\mSigma$.
Then the Fisher information matrix at $\rvs$ is
\begin{align*}
    \mI(\rvs)=\nabla_\rvs\vmu(\rvs)^\top\mSigma^{-1}\nabla_\rvs\vmu(\rvs).
\end{align*}
From this expression, we see that the discrimination threshold will depend on how the mean response is changing in the direction $\vepsilon$ relative to the noise covariance.

\section{Optimal distortions of image representations}

Given estimates of discrimination thresholds based on image representations, one can compare them with human discrimination thresholds to gain insights into the similarities and differences between image representations and human perceptual systems.
However, measuring human discrimination thresholds is expensive. 
For example, \citet{macadam1942visual} mapped out human perceptual thresholds in two-dimensional color space, which involved approximately 25,000 experimental trials for each observer.
This was a monumental effort in two-dimensions and the dimensions of photographic images are orders of magnitude larger, making comprehensive perceptual discrimination measurements infeasible.
Rather, we must select only a handful of image distortions for comparison.
How should we choose these distortions to decide which model best captures human discrimination thresholds?

In the following, we review existing approaches for optimally choosing image distortions for evaluating a single image representations \citep{berardino2017eigen} or directly comparing two image representations \citep{zhou2024comparing}.
We then propose a general method for optimally choosing distortions when comparing any number of image representations, including continuous families of image representations.

\subsection{Eigen-distortions of an image representation}

Suppose we have a single image representation $p(\rvr|\rvs)$.
For a given image $\rvs$, \citet{berardino2017eigen} proposed comparing the distortions with the largest- and smallest- predicted discrimination thresholds.
These are the distortions $\vepsilon_\text{max}(\rvs)$ and $\vepsilon_\text{min}(\rvs)$ that maximize and minimize the thresholds, which correspond to the extremal eigenvectors of the Fisher information matrix $\mI(\rvs)$.
Fittingly, they referred to these distortions as ``eigen-distortions''.

After computing the eigen-distortions $\vepsilon_\text{max}(\rvs)$ and $\vepsilon_\text{min}(\rvs)$, Berardino et al.\ measured human discrimination thresholds $t_\text{human}(\rvs;\vepsilon_\text{max})$ and $t_\text{human}(\rvs;\vepsilon_\text{min})$ and proposed the ratio between these thresholds
\begin{align*}
    r=\log \frac{t_\text{human}(\rvs;\vepsilon_\text{max}(\rvs))}{t_\text{human}(\rvs;\vepsilon_\text{min}(\rvs))}
\end{align*}
as a measure of how well a model predicts human discrimination thresholds.
The larger the ratio $r$, the better the model predicts (extremal) human discrimination thresholds.

While this is sensible when evaluating a single image representation, it may not be optimal when comparing two representations.
For example, two image representations may have similar extremal distortions and still generate vastly different perceptual predictions in response to non-extremal distortions.
If the goal is to find the distortions that maximally \textit{differentiate} the image representations, computing the eigen-distortions for each image representation will not necessarily provide insight into the differences between the models.

\subsection{Generalized eigen-distortions for comparing two image representations}

Consider the case we're comparing two image representations $p_A(\rvr_A|\rvs)$ and $p_B(\rvr_B|\rvs)$.
\citet{zhou2024comparing} proposed choosing distortions $\vepsilon$ in which the predicted discrimination thresholds maximally differ and testing these distortions against human perceptual discriminability.
Specifically, they proposed choosing the distortions $\vepsilon$ that maximize the ratios of the discrimination thresholds between the two models:
\begin{align*}
    \vepsilon_{A/B}(\rvs)=\argmax_\vepsilon\frac{t_A(\rvs;\vepsilon)}{t_B(\rvs;\vepsilon)},&&\vepsilon_{B/A}(\rvs)=\argmax_\vepsilon\frac{t_B(\rvs;\vepsilon)}{t_A(\rvs;\vepsilon)}.
\end{align*}
These distortions are natural generalizations of eigen-distortions.
For instance, in the special case that $\mI_B(\rvs)$ is the identity matrix, which corresponds to an image representation that is equally sensitive to all distortions, $\vepsilon_{A/B}(\rvs)$ and $\vepsilon_{B/A}(\rvs)$ correspond to the eigen-distortions of image representation $p_A(\rvr_A|\rvs)$.
For general $\mI_B(\rvs)$, the distortions $\vepsilon_{A/B}(\rvs)$ and $\vepsilon_{B/A}(\rvs)$ correspond to the extremal eigenvectors of the generalized eigenvalue problem $\mI_A(\rvs)\vepsilon=\lambda\mI_B(\rvs)\vepsilon$,
so we refer to them as ``generalized eigen-distortions''. 


% While this example may seem artificial, it is perhaps not so unreasonable.
% In particular, this example captures subtleties that can arise when comparing two models with the same mean responses but different noise statistics.

% From this example, we see that only comparing which threshold is larger can lead to counter-intuitive results. 
% Rather, we can accurately judge which model better predicts human discrimination thresholds along distortion $\vepsilon_{A/B}$ and $\vepsilon_{B/A}$ by comparing the log ratios between the thresholds.

\subsection{Principal distortions for comparing multiple image representations}

Given any two distortions $\vepsilon_1$ and $\vepsilon_2$, we can define a metric on image representations (at $\rvs$) that is only in terms of (estimated) discrimination thresholds in the directions of these distortions:
\begin{align}\label{eq:metric}
    d_{\vepsilon_1,\vepsilon_2}(A,B):=\left|\log \frac{t_A(\vs;\vepsilon_1)}{t_A(\vs;\vepsilon_2)}-\log \frac{t_B(\vs;\vepsilon_1)}{t_B(\vs;\vepsilon_2)}\right|.
\end{align}
Essentially, we map the discrimination thresholds to their log ratio and then compute the difference.
This metric has some appealing properties.
First, it is invariant to arbitrary scaling of the Fisher information matrix.
Second, it is invariant to permutations of $\vepsilon_1$ and $\vepsilon_2$.
Third, the metric can be derived as an approximation of the affine invariant Riemannian metric on positive definite matrices, and this allows for a natural extension to defining the metric when there are more than 2 thresholds (Appx.~\ref{apdx:metric}).
Using this metric we can evaluate which model is closer to human representations.
Specifically, image representation $A$ is the better predictor if $d(A,\text{human})<d(B,\text{human})$ and vice versa.

Suppose we have a family of image representations.
How should we choose the top two distortions?

We first formulate a compact optimization problem for the generalized eigen-distortions from the previous section.
Given two image representations, we can express the generalized eigen-distortions as solution to the optimization problem
\begin{align}\label{eq:pairwise-optimization}
    \{\vepsilon_{A/B}(\rvs),\vepsilon_{B/A}(\rvs)\}=\argmax_{\vepsilon_1,\vepsilon_2}d_{\vepsilon_1,\vepsilon_2}(A,B).
\end{align}
From these expression, we see that the generalized eigen-distortions are chosen to maximize the \textit{difference} between the log ratios of the thresholds.
% The eigen-distortion are a special case of the generalized eigen-distortions when image representation $B$ has a threshold function that is constant in $\vepsilon$.
Given $N$ image representations, the above expression can be generalized by maximizing the sum of the squares of all pairwise differences between the log ratios of the thresholds, which is equivalent to maximizing the variance of the log ratios of the thresholds.
In particular, given a family of image representations indexed by $\theta$ and a probability distribution over image representations $p(\theta)$, we can express the optimal distortions as solutions of the following optimization problem
\begin{align}\label{eq:variance}
    \{\vepsilon_1(\rvs),\vepsilon_2(\rvs)\} &=\argmax_{\vepsilon_1,\vepsilon_2}\text{Var}_{\theta\sim p(\theta)}\left\{\log\frac{t_\theta(\rvs;\vepsilon_1)}{t_\theta(\rvs;\vepsilon_2)}\right\}.
\end{align}
There is also a natural generalization to finding the top $K$ distortions.
For a gradient-based optimization algorithm, see Appendix \ref{apdx:algorithm}.

Given distortions $\{\vepsilon_1,\vepsilon_2\}$, we can define a metric between two image representations in terms of \eqref{eq:metric}.
% \begin{align*}
%     d^2(A,B)&=\sum_{j=1}^K\sum_{k=1}^K\left\{\log \frac{t_A(\vs;\vepsilon_k)}{t_B(\vs;\vepsilon_k)}-\log \frac{t_A(\vs;\vepsilon_j)}{t_B(\vs;\vepsilon_j)}\right\}^2\\
%     &=\sum_{k=1}^K\left\{\log \frac{t_A(\vs;\vepsilon_k)}{t_B(\vs;\vepsilon_k)}-\frac1K\sum_{j=1}^K\log \frac{t_A(\vs;\vepsilon_j)}{t_B(\vs;\vepsilon_j)}\right\}^2\\
%     &=\text{Var}_{\vepsilon\sim\text{Unif}(\vepsilon_1,\dots,\vepsilon_K)}\left\{\log\frac{t_A(\rvs;\vepsilon)}{t_B(\rvs;\vepsilon)}\right\}.
% \end{align*}
% \begin{align*}
%     d^2(A,B)&=\left\{\log \frac{t_A(\vs;\vepsilon_1)}{t_B(\vs;\vepsilon_1)}-\log \frac{t_A(\vs;\vepsilon_2)}{t_B(\vs;\vepsilon_2)}\right\}^2.
% \end{align*}
A threshold is essentially the width of a slice through the ellipsoid corresponding to the inverse Fisher information matrix.
Therefore, this metric can be interpreted as comparing two inverse Fisher information matrices by comparing the (log) ratios of widths in the directions $\vepsilon_1$ and $\vepsilon_2$.
For more on this metric and its relationship to the affine invariant Riemannian manifold on positive definite matrices, see Appendix \ref{apdx:metric}.

\section{Experiments}

% \subsection{Local linearity of deep nets}

% How well does a local linear approximation of a deep network approximate its input-output function $\vmu(\cdot)$?
% Given $\rvs$ and $\vepsilon$, define
% \begin{align*}
%     h(\alpha):=\left\|\frac{\vmu(\rvs+\alpha\vepsilon)-\vmu(\rvs)}{\alpha}-\nabla_\rvs\vmu(\rvs)\vepsilon\right\|.
% \end{align*}
% Then $h(\alpha)=0$ for $\alpha$ sufficiently small. 
% Plots of $h(\alpha)$.

% \subsection{Synthetic data}

% Consider a three-dimensional stimulus $\rvs$ and a family of models indexed by $\theta\in\Theta$ with uniform prior $p(\theta)$ and corresponding \textit{diagonal} Fisher information matrices $\{\mI_\theta(\rvs)\}$.
% In this case, we can express each Fisher information matrix as
% \begin{align*}
%     \mI_\theta(\rvs)=\mLambda(\theta)=\text{diag}(\lambda_1(\theta),\lambda_2(\theta)),
% \end{align*}
% and the threshold function as
% \begin{align*}
%     t_\theta(\rvs;\vepsilon)&=\sqrt{\lambda_1(\theta)\epsilon_1^2+\lambda_2(\theta)\epsilon_2^2}.
% \end{align*}
% and the log ratio as
% \begin{align*}
%     \log\frac{t_\theta(\rvs;\vepsilon_1)}{t_\theta(\rvs;\vepsilon_2)}&=\log\frac{\lambda_1(\theta)}{\lambda_2(\theta)}.
% \end{align*}

% \subsection{Toy example}

% Let
% \begin{align*}
%     \mA&=\text{diag}(e^3,e^2,e^4)\\
%     \mB&=\text{diag}(e^5,1,e^4)\\
%     \mC&=\text{diag}(e^5,e^2,e^{-1}).
% \end{align*}
% The optimal directions when comparing $\mA$ versus $\mB$ are $\ve_1$ and $\ve_2$.
% The optimal directions when comparing $\mA$ versus $\mC$ are $\ve_1$ and $\ve_3$.
% The optimal directions when comparing $\mB$ versus $\mC$ are $\ve_2$ and $\ve_3$.
% The eigen-distortions of $\mA$ are $\ve_2$ and $\ve_3$, the eigen-distortions of $\mB$ are $\ve_1$ and $\ve_2$, and the eigen-distortions of $\mC$ are $\ve_1$ and $\ve_3$.

% What is the affine-invariant Riemannian distance between these matrices?
% \begin{align*}
%     d(\mA,\mB)&=\sqrt{3\text{Var}\{-2,2,0\}}=\sqrt{3(2^2+2^2)}=2\sqrt{6}\\
%     d(\mA,\mC)&=\sqrt{3\text{Var}\{-2,0,5\}}=\sqrt{3(3^2+1^2+4^2)}=\sqrt{78}\\
%     d(\mB,\mC)&=\sqrt{3\text{Var}\{0,-2,5\}}=\sqrt{3(1^2+3^2+4^2)}=\sqrt{78}.    
% \end{align*}

% What are the optimal 2 directions when comparing all 3 at once?

% Note that
% \begin{align*}
%     \vw^\top\mA\vw&=e^2(ew_1^2+w_2^2+e^2w_3^2)\\
%     \vw^\top\mB\vw&=e^5w_1^2+w_2^2+e^4w_3^2\\
%     \vw^\top\mC\vw&=e^{-1}(e^4w_1^2+e^3w_2^2+w_3^2).
% \end{align*}
% Given $\vepsilon_1$ and $\vepsilon_2$,
% \begin{align*}
%     g_1(\vepsilon_1,\vepsilon_2)=\frac12\log\frac{\vepsilon_1^\top\mA\vepsilon_1}{\vepsilon_2^\top\mA\vepsilon_2}&=\frac12\log\frac{e\epsilon_{11}^2+\epsilon_{12}^2+e^2\epsilon_{13}^2}{e\epsilon_{21}^2+\epsilon_{22}^2+e^2\epsilon_{23}^2}\\
%     g_2(\vepsilon_1,\vepsilon_2)=\frac12\log\frac{\vepsilon_1^\top\mB\vepsilon_1}{\vepsilon_2^\top\mB\vepsilon_2}&=\frac12\log\frac{e^5\epsilon_{11}^2+\epsilon_{12}^2+e^4\epsilon_{13}^2}{e^5\epsilon_{21}^2+\epsilon_{22}^2+e^4\epsilon_{23}^2}\\
%     g_3(\vepsilon_1,\vepsilon_2)=\frac12\log\frac{\vepsilon_1^\top\mC\vepsilon_1}{\vepsilon_2^\top\mC\vepsilon_2}&=\frac12\log\frac{e^4\epsilon_{11}^2+e^3\epsilon_{12}^2+\epsilon_{13}^2}{e^4\epsilon_{21}^2+e^3\epsilon_{22}^2+\epsilon_{23}^2}
% \end{align*}
% The optimization problem is
% \begin{align*}
%     \max_{\vepsilon_1,\vepsilon_2}\sum_{n=1}^3\left\{g_n(\vepsilon_1,\vepsilon_2)-\frac13\sum_{m=1}^3g_m(\vepsilon_1,\vepsilon_2)\right\}^2
% \end{align*}

\subsection{Distortions that differentiate models of color vision deficiency}

Human normal color vision requires large (L), medium (M) and short (S) cones (photoreceptors) with different spectral sensitivities.
The absence of a cone type or variations in a cone type's spectral sensitivity affects an individual's color perception and, consequently, their ability to perform certain visual tasks.
Therefore, better understanding the differences between individuals with various color vision deficiencies has potential practical implications.

Using our method, we estimate color distortions that differentiate several models of color vision deficiency in terms of their perceptual discriminability thresholds.
Specifically, we consider stochastic color representations for nine types of color vision deficiency in addition to normal color vision, resulting in a total of $N=10$ color representations.
We assume that a color can be encoded as a three-dimensional vector $\rvs\in\R^3$ in RGB space, which captures the range of stimuli that can be produced by most electronic displays.
For each model $n=1,\dots,10$, we assume there is a (deterministic) function $\vf_n:\R^3\mapsto\R^3$ that maps the stimulus $\rvs$ to a vector of large, medium and short (LMS) cone responses $\rvc=\vf_n(\rvs)+\rvn$, where $\rvn$ is isotropic Gaussian noise. 
% \citep{machado2009physiologically}.
The cone responses $\rvc$ are then mapped to a stochastic representation $\rvr=\rvp(\vg(\rvc))$, where $\vg:\R^3\mapsto\R^D$ is a function that is fixed across models and $\rvp$ is a Poisson process.
% \citep{Carter2018CIE0C}
Note that this is a strong simplification that assumes the processing of cone responses by downstream brain areas does not depend on an individual's cone properties.
While this is likely false since neural systems are highly adaptive, it serves as a reasonable starting point for testing our method.
With these simplifications, and assuming that $\vf$ and $\vg$ are linear, the $n$\textsuperscript{th} model's discrimination prediction at stimulus $\rvs\in\R^3$ to distortion $\vepsilon\in\R^3$ is
\begin{align*}
    d(\rvs;\vepsilon)=\sqrt{\vepsilon^\top\nabla\vf_n(\rvs)^\top\nabla\vg(\vf_n(\rvs))^\top\nabla\vg(\vf_n(\rvs))\nabla\vf_n(\rvs)\vepsilon}.
\end{align*}
For a given stimulus $\rvs$, we compute the distortions $\vepsilon$ that maximize the variance in \eqref{eq:variance}.
To compute the variance, we can assume that the probability of each model is either equal---i.e., $p(n)=1/N$---or given by the proportion of individuals affected by that type of color deficiency.

\subsection{Early visual models}

\subsection{Deep neural networks}

\section{Discussion}

Related work: local information geometry of retinal representations \citep{ding2023information}.
